Faster than Fast: Accelerating the Griffin-Lim Algorithm

The phase retrieval problem is found in various areas of applications of engineering and applied physics. It is also a very active field of research in mathematics, signal processing and machine learning. In this paper, we present an accelerated version of the well known Fast Griffin-Lim algorithm (FGLA) for the phase retrieval problem in a general setting. It has increased the speed of convergence, and most importantly, the limit points of the generated sequence can reach a significantly smaller error than the ones generated by FGLA. We will give a motivation of the acceleration and compare it numerically to its predecessors and other algorithms typically used to solve similar problems.

==> Literature.tex <==
https://publik.tuwien.ac.at/files/publik_253102.pdf
> Oversampled

https://arxiv.org/pdf/1508.02820.pdf
> IEE Article
